T\"oRF: Time-of-Flight Radiance Fields for Dynamic Scene View Synthesis

Neural networks can represent and accurately reconstruct radiance fields for static 3D scenes (e.g., NeRF). Several works extend these to dynamic scenes captured with monocular video, with promising performance. However, the monocular setting is known to be an under-constrained problem, and so methods rely on data-driven priors for reconstructing dynamic content. We replace these priors with measurements from a time-of-flight (ToF) camera, and introduce a neural representation based on an image formation model for continuous-wave ToF cameras. Instead of working with processed depth maps, we model the raw ToF sensor measurements to improve reconstruction quality and avoid issues with low reflectance regions, multi-path interference, and a sensor's limited unambiguous depth range. We show that this approach improves robustness of dynamic scene reconstruction to erroneous calibration and large motions, and discuss the benefits and limitations of integrating RGB+ToF sensors that are now available on modern smartphones.

==> figures/figure4_staticqualitative/fig04_staticqualitative.tex <==
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccccc}
    & 2-view NVS & 2-view depth & 4-view NVS & 4-view depth \\
    \rotatebox{90}{\footnotesize~~~~~(a) NeRF~\cite{MildeSTBRN2020}} &
    \includegraphics[width=1.33in,height=1in]{figures/figure4_staticqualitative/color_nerf_2.png} &
    \includegraphics[decodearray={0.0 1.5 0.0 1.5 0.0 1.0},width=1.33in,height=1in]{figures/figure4_staticqualitative/disp_colormap/bathroom_disparity_nerf_2.png} &
    \includegraphics[width=1.33in,height=1in]{figures/figure4_staticqualitative/color_nerf_4.png} &
    \includegraphics[decodearray={0.0 1.5 0.0 1.5 0.0 1.0},width=1.33in,height=1in]{figures/figure4_staticqualitative/disp_colormap/bathroom_disparity_nerf_4.png} \\
    % & \multicolumn{4}{c}{(a) NeRF~\cite{MildeSTBRN2020} (left to right: 2-view NVS, 2-view depth, 4-view NVS, 4-view depth)}\\
    \rotatebox{90}{~~~\footnotesize(d) \torf (ours)} &
    % &
    \includegraphics[width=1.33in,height=1in]{figures/figure4_staticqualitative/color_ours_2.png} &
    \includegraphics[decodearray={0.0 1.5 0.0 1.5 0.0 1.0},width=1.33in,height=1in]{figures/figure4_staticqualitative/disp_colormap/bathroom_disparity_ours_2.png} &
    \includegraphics[width=1.33in,height=1in]{figures/figure4_staticqualitative/color_ours_4.png} &
    \includegraphics[decodearray={0.0 1.5 0.0 1.5 0.0 1.0},width=1.33in,height=1in]{figures/figure4_staticqualitative/disp_colormap/bathroom_disparity_ours_4.png} \\
    % & \multicolumn{4}{c}{(b) \torf (ours)  (left to right: 2-view NVS, 2-view depth, 4-view NVS, 4-view depth)}
    \end{tabular}
    \caption{\emph{Adding ToF aids reconstruction for low numbers of views.}
    In the classic multi-view static setting, NeRF quality suffers as the number of views decreases.
    For two RGB views, adding ToF data makes view synthesis possible.
    For four RGB views, ToF data increases depth quality over NeRF.
    Note the clean depth with sharp edges and fine geometric details such as the lamps above the mirror.
    %\jt{What is interesting about this experiment? How the depth improves over derived raw?}
    }
    \label{fig:comparison-few-views}
\end{figure}

==> figures/figure5_dynamicqualitative/fig05_dino_estimated.tex <==
\begin{figure}%[p]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    %\newcommand{\rgbcolormap}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\imgw}{1.31in}
    \newcommand{\imgh}{1in}
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[decodearray=\rgbcolormap,width=\imgw,height=\imgh,trim=#1,clip]{figures/#2}}
    
    \newcommand{\zoomRGB}[4]{
    \begin{tikzpicture}[
		image/.style={inner sep=0pt, outer sep=0pt},
		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
		style1/.style={cyan!90!black,thick},
		style2/.style={orange!90!black},
		style3/.style={blue!90!black},
		style4/.style={green!90!black},
		style5/.style={white},
		style6/.style={black},
    ]
    
    \node [image] (#1) {\includegraphics[width=\imgw,height=\imgh]{#2}};
    \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
    
    \end{tikzpicture}
    }
    
    \begin{tabular}{c c@{\hspace{0.2mm}}c@{\hspace{0.2mm}}c@{\hspace{0.2mm}}c}
    
    % Legend
    &
    (a) Input &
    (b) NSFF & 
    (c) VideoNeRF &
    (d) \torf (Ours) \\
    
    % DinoPear RGB
    \multirow{2}{*}[1em]{\rotatebox{90}{\footnotesize DinoPear}} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/input_rgb.mp4.jpg}{(-0.55,0.3)}{south west} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/nsff_rgb.mp4.jpg}{(-0.7,0.3)}{south west} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/cvd_rgb.png}{(-0.7,0.3)}{south west} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/torf_rgb.mp4.jpg}{(-0.5,0.25)}{south west} \\[-1pt]
    
    % DinoPear Depth
    &
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/input_tof.mp4.jpg}{(-0.55,0.3)}{south west} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/nsff_depth.mp4.jpg}{(-0.7,0.3)}{south west} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/cvd_depth.png}{(-0.7,0.3)}{south west} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/torf_depth.mp4.jpg}{(-0.5,0.25)}{south west} \\[-1pt]

    \end{tabular}
    
    \caption{\emph{Adding ToF supervision helps improve quality.}
    Compared to two video baselines, Video\-NeRF~\citep{XianHKK2021} (modified to use ToF-derived depth) and NSFF~\citep{LiNSW2021}, our approach reduces errors in static scene components and some dynamic components.
    % Top to bottom: Novel views from \SeqStudyBook, \SeqDishwasher, and \SeqDinoPear.
    All models were trained for comparable times.
    Please see \href{https://imaging.cs.cmu.edu/torf}{our website} for video comparisons.
	}
    \label{fig:comparison-dynamic2-dino-estimated}
\end{figure}

==> figures/figure5_dynamicqualitative/fig05_dino_nowrap.tex <==
\begin{figure}%[p]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    %\newcommand{\rgbcolormap}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\imgw}{1.31in}
    \newcommand{\imgh}{1in}
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[decodearray=\rgbcolormap,width=\imgw,height=\imgh,trim=#1,clip]{figures/#2}}
    
    \newcommand{\zoomRGB}[4]{
    \begin{tikzpicture}[
		image/.style={inner sep=0pt, outer sep=0pt},
		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
		style1/.style={cyan!90!black,thick},
		style2/.style={orange!90!black},
		style3/.style={blue!90!black},
		style4/.style={green!90!black},
		style5/.style={white},
		style6/.style={black},
    ]
    
    \node [image] (#1) {\includegraphics[width=\imgw,height=\imgh]{#2}};
    \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
    
    \end{tikzpicture}
    }
    
    \begin{tabular}{c c@{\hspace{0.2mm}}c@{\hspace{0.2mm}}c@{\hspace{0.2mm}}c}
    
    % Legend
    &
    (a) Input &
    (b) NSFF+ToF & 
    (c) VideoNeRF+ToF &
    (d) \torf (Ours) \\
    
    % DinoPear RGB
    \multirow{2}{*}[3em]{\rotatebox{90}{\footnotesize DinoPear unwrapped}} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/input_rgb.mp4.jpg}{(0.325,-0.1)}{south east} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/nsff_tof_rgb.png}{(0.45,-0.075)}{south east} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/videonerf_nowrap_rgb.png}{(0.45,-0.075)}{south east} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/torf_rgb.mp4.jpg}{(0.35,-0.1)}{south east} \\[-1pt]
    
    % DinoPear Depth
    &
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/input_nowrap_depth.png}{(0.325,-0.1)}{south east} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/nsff_tof_depth.png}{(0.45,-0.075)}{south east} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/videonerf_nowrap_depth.png}{(0.45,-0.075)}{south east} &
    
    \zoomRGB{nsff-rgb-phonebooth}{figures/figure5_dynamicqualitative/dinopear/torf_depth.mp4.jpg}{(0.35,-0.1)}{south east} \\[-1pt]

    \end{tabular}
    
    \caption{\emph{Adding ToF supervision helps improve quality.}
    Compared to two video baselines, Video\-NeRF~\citep{XianHKK2021} (modified to use ToF-derived depth) and NSFF~\citep{LiNSW2021}, our approach reduces errors in static scene components and some dynamic components.
    % Top to bottom: Novel views from \SeqStudyBook, \SeqDishwasher, and \SeqDinoPear.
    All models were trained for comparable times.
    Please see \href{https://imaging.cs.cmu.edu/torf}{our website} for video comparisons.
	}
    \label{fig:comparison-dynamic2-dino-nowrap}
\end{figure}

==> figures/figure7_rawtofvsdepth/fig07_rawtofvsdepth_neurips.tex <==
\begin{figure}[t]
    \def\imgwidth{0.243\linewidth}
    % \vspace{-\baselineskip}
    \centering
    \begin{tikzpicture}[
		image/.style={inner sep=0pt, outer sep=0pt},
		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
		spy using outlines={rectangle, size=1.5cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
		style1/.style={cyan!90!black,thick},
		style2/.style={orange!90!black},
		style3/.style={blue!90!black},
		style4/.style={green!90!black},
	]
	
	\def\padding{2pt}
	% decodearray here is used to remap RGB values in the image to new limits, which we use to brighten the image overall.
    % 	\newcommand{\subfigRGB}[2][0 0 0 0]{\includegraphics[decodearray={0.2 1.2 0.2 1.2 0.2 1.2},width=\imgwidth,trim=#1,clip]{figures/#2.png}}
    % 	\newcommand{\subfigDepth}[2][0 0 0 0]{\includegraphics[width=\imgwidth,trim=#1,clip]{figures/#2.png}}
    %     \newcommand{\subfigDepthTwo}[2][0 0 0 0]{\includegraphics[decodearray={0.0 2.0 0.0 2.0 0.0 2.0},width=\imgwidth,trim=#1,clip]{figures/#2.png}}
    
    \newcommand{\subfigRGB}[2][0 0 0 0]{\includegraphics[decodearray={0.2 1.2 0.2 1.2 0.2 1.2},width=\imgwidth,trim=#1,clip]{figures/#2.png}}
	\newcommand{\subfigDepth}[2][0 0 0 0]{\includegraphics[width=\imgwidth,trim=#1,clip]{figures/#2.png}}
    \newcommand{\subfigDepthTwo}[2][0 0 0 0]{\includegraphics[width=\imgwidth,trim=#1,clip]{figures/#2.png}}

	% Left two
    % 	\node [image] (rgb-photocopier) at (0, 0) {\subfigRGB{figure7_rawtofvsdepth/videonerf_photocopier_depthwrap_rgb}};
    % 	\node [image,right=\padding] (depth-photocopier) at (rgb-photocopier.east) {\subfigDepth{figure7_rawtofvsdepth/videonerf_photocopier_depthwrap_depth}};
    \node [image] (rgb-photocopier) at (0, 0) {\subfigRGB{figure5_dynamicqualitative/videonerf/copier_015_color}};
	\node [image,right=\padding] (depth-photocopier) at (rgb-photocopier.east) {\subfigDepth{figure5_dynamicqualitative/videonerf/copier_015_depth}};

    % Right two
	\node [image,right=4pt] (rgb-studybook) at (depth-photocopier.east) {\subfigRGB[20 20 20 10]{figure7_rawtofvsdepth/torf_photocopier_depthwrap_rgb}};
	\node [image,right=\padding] (depth-studybook) at (rgb-studybook.east) {\subfigDepthTwo[20 20 20 10]{figure7_rawtofvsdepth/torf_photocopier_depthwrap_depth_magmahack3}};

    % Top row cut out
	\spy[style3] on ($(rgb-photocopier.center)-(-1.25,-0.9)$) in node (crop-rgb-photocopier) [anchor=south west] at (rgb-photocopier.south west);
	\spy[style3] on ($(depth-photocopier.center)-(-1.25,-0.9)$) in node (crop-depth-photocopier) [anchor=south west] at (depth-photocopier.south west);
	
	% Bottom row cut out
	\spy[style3] on ($(rgb-studybook.center)-(-1.25,-0.9)$) in node (crop-rgb-studybook) [anchor=south west] at (rgb-studybook.south west);
	\spy[style3] on ($(depth-studybook.center)-(-1.25,-0.9)$) in node (crop-depth-studybook) [anchor=south west] at (depth-studybook.south west);

    % Labels
	\node [collabel] at (rgb-photocopier.north)  {\small Depth supervision (NVS)};
	\node [collabel] at (depth-photocopier.north)  {\small Volume depth};
	\node [collabel] at (rgb-studybook.north)  {\small Phasor supervision (NVS)};
	\node [collabel] at (depth-studybook.north)  {\small Volume depth};
	
	\end{tikzpicture}
	\caption{\emph{Raw phasor supervision improves reconstruction.} Wrap-around phase bounds the range of useful ToF measurements when depth is derived first and used as supervision (left). Our approach of modeling raw phasor measurements within the neural volume alleviates this problem (right). %\jt{Scene depth scale is off; low priority fix}
	}
	\label{fig:rawtofvsdepth}
\end{figure}

==> figures/raw_brisque.tex <==
\begin{tabular}{ll}
\toprule
                                                                             filename & BRISQUE_score \\
\midrule
% MP4s for RGB
                                         ToRF_Results/NSFF/DeskBox_NSFF_spiral_15.mp4 &    46.4 $\pm$ 2.4 \\
                                        ToRF_Results/NSFF/Cupboard_NSFF_spiral_15.mp4 &    32.7 $\pm$ 1.5 \\
                                      ToRF_Results/NSFF/PhoneBooth_NSFF_spiral_15.mp4 &    42.2 $\pm$ 1.3 \\
                                     ToRF_Results/NSFF/Photocopier_NSFF_spiral_15.mp4 &    42.0 $\pm$ 2.3 \\
                                       ToRF_Results/NSFF/StudyBook_NSFF_spiral_15.mp4 &    40.4 $\pm$ 2.5 \\
                                               ToRF_Results/NSFF/Dishwasher_NSFF_.mp4 &    21.9 $\pm$ 3.3 \\

                                         ToRF_Results/ToRF/DeskBox_ToRF_spiral_15.mp4 &    27.9 $\pm$ 2.3 \\
                                        ToRF_Results/ToRF/Cupboard_ToRF_spiral_15.mp4 &    25.7 $\pm$ 1.4 \\
                                      ToRF_Results/ToRF/PhoneBooth_ToRF_spiral_15.mp4 &    28.4 $\pm$ 1.2 \\
                                     ToRF_Results/ToRF/Photocopier_ToRF_spiral_15.mp4 &    28.6 $\pm$ 2.5 \\
                                       ToRF_Results/ToRF/StudyBook_ToRF_spiral_15.mp4 &    25.8 $\pm$ 2.0 \\
                                               ToRF_Results/ToRF/Dino_ToRF_spiral.mp4 &    18.8 $\pm$ 1.7 \\
  ToRF_Results/ToRF/ios_dishwasher_clean_30_dynamic_fast_spiral_00200000_radiance.mp4 &    25.8 $\pm$ 1.9 \\
ToRF_Results/ToRF/real_seq_color21_small_30_dynamic_fast_spiral_00140001_radiance.mp4 &    32.6 $\pm$ 1.2 \\

                                ToRF_Results/NeRF/package/package_static_nerf_10k.mp4 &    29.4 $\pm$ 2.7 \\
                                               ToRF_Results/NeRF/phonebooth/video.mp4 &    33.2 $\pm$ 5.7 \\
                                 
% Disparity maps                                    
                                    ToRF_Results/ToRF/DeskBox_ToRF_spiral_15_disp.mp4 &    60.6 $\pm$ 1.1 \\
                                     ToRF_Results/ToRF/Copier_ToRF_spiral_15_disp.mp4 &    58.6 $\pm$ 1.3 \\
                                   ToRF_Results/ToRF/Cupboard_ToRF_spiral_15_disp.mp4 &    60.6 $\pm$ 1.8 \\
                                 ToRF_Results/ToRF/PhoneBooth_ToRF_spiral_15_disp.mp4 &    65.8 $\pm$ 0.9 \\      ToRF_Results/ToRF/StudyBook_ToRF_spiral_15_disp.mp4 &    73.4 $\pm$ 1.1 \\
      ToRF_Results/ToRF/ios_dishwasher_clean_30_dynamic_fast_spiral_00200000_disp.mp4 &    50.7 $\pm$ 2.4 \\
    ToRF_Results/ToRF/real_seq_color21_small_30_dynamic_fast_spiral_00140001_disp.mp4 &    67.4 $\pm$ 0.9 \\
                                          ToRF_Results/ToRF/Dino_ToRF_spiral_disp.mp4 &    52.6 $\pm$ 1.7 \\
                                          


% OLD VideoNeRF numbers
                                   ToRF_Results/VideoNeRF/dino_dynamic/disp_0_449.mp4 &    52.2 $\pm$ 1.4 \\
                                     ToRF_Results/VideoNeRF/dishwasher/disp_0_449.mp4 &    54.0 $\pm$ 1.0 \\
                                      ToRF_Results/VideoNeRF/warped_21/disp_0_449.mp4 &    59.2 $\pm$ 5.8 \\
                                      ToRF_Results/VideoNeRF/warped_22/disp_0_449.mp4 &    63.8 $\pm$ 1.4 \\
                                      ToRF_Results/VideoNeRF/warped_24/disp_0_449.mp4 &    64.0 $\pm$ 0.6 \\
                                      ToRF_Results/VideoNeRF/warped_26/disp_0_449.mp4 &    44.7 $\pm$ 1.7 \\
                                  ToRF_Results/VideoNeRF/dino_dynamic/video_0_449.mp4 &    48.4 $\pm$ 1.5 \\
                                    ToRF_Results/VideoNeRF/dishwasher/video_0_449.mp4 &    31.2 $\pm$ 0.8 \\
                                     ToRF_Results/VideoNeRF/warped_21/video_0_449.mp4 &    48.7 $\pm$ 0.6 \\
                                     ToRF_Results/VideoNeRF/warped_22/video_0_449.mp4 &    44.6 $\pm$ 0.5 \\
                                     ToRF_Results/VideoNeRF/warped_24/video_0_449.mp4 &    49.4 $\pm$ 0.6 \\
                                     ToRF_Results/VideoNeRF/warped_26/video_0_449.mp4 &    41.6 $\pm$ 0.7 \\
%
%
% PNGs 
                                                           ToRF_Results/NeRF/cupboard &    27.9 $\pm$ 1.9 \\
                                                            ToRF_Results/NeRF/package &    33.0 $\pm$ 2.9 \\
                                                         ToRF_Results/NeRF/phonebooth &    34.2 $\pm$ 7.2 \\
                                     ToRF_Results/NSFF/Cupboard_NSFF_spiral_15/depths &    36.1 $\pm$ 3.6 \\
                                   ToRF_Results/NSFF/PhoneBooth_NSFF_spiral_15/depths &    41.4 $\pm$ 2.5 \\
                                  ToRF_Results/NSFF/Photocopier_NSFF_spiral_15/depths &    39.9 $\pm$ 2.9 \\
                                    ToRF_Results/NSFF/StudyBook_NSFF_spiral_15/depths &    33.5 $\pm$ 4.2 \\
                            ToRF_Results/NSFF/Cupboard_NSFF_spiral_15/depths_colormap &    31.6 $\pm$ 3.4 \\
                          ToRF_Results/NSFF/PhoneBooth_NSFF_spiral_15/depths_colormap &    37.0 $\pm$ 2.5 \\
                         ToRF_Results/NSFF/Photocopier_NSFF_spiral_15/depths_colormap &    34.9 $\pm$ 2.8 \\
                           ToRF_Results/NSFF/StudyBook_NSFF_spiral_15/depths_colormap &    30.4 $\pm$ 3.8 \\
                                     ToRF_Results/NSFF/Cupboard_NSFF_spiral_15/images &    28.1 $\pm$ 2.5 \\
                                   ToRF_Results/NSFF/PhoneBooth_NSFF_spiral_15/images &    37.0 $\pm$ 2.0 \\
                                  ToRF_Results/NSFF/Photocopier_NSFF_spiral_15/images &    36.6 $\pm$ 3.3 \\
                                    ToRF_Results/NSFF/StudyBook_NSFF_spiral_15/images &    34.2 $\pm$ 4.3 \\
% OLD VideoNeRF numbers
                                            ToRF_Results/VideoNeRF/dino_dynamic/disps &    78.5 $\pm$ 0.7 \\
                                              ToRF_Results/VideoNeRF/dishwasher/disps &    71.6 $\pm$ 0.6 \\
                                               ToRF_Results/VideoNeRF/warped_21/disps &    83.1 $\pm$ 8.0 \\
                                               ToRF_Results/VideoNeRF/warped_22/disps &    89.4 $\pm$ 0.3 \\
                                               ToRF_Results/VideoNeRF/warped_24/disps &    83.1 $\pm$ 0.3 \\
                                               ToRF_Results/VideoNeRF/warped_26/disps &    60.9 $\pm$ 0.5 \\
                                           ToRF_Results/VideoNeRF/dino_dynamic/images &    58.1 $\pm$ 1.9 \\
                                             ToRF_Results/VideoNeRF/dishwasher/images &    34.3 $\pm$ 0.6 \\
                                              ToRF_Results/VideoNeRF/warped_21/images &    56.8 $\pm$ 0.4 \\
                                              ToRF_Results/VideoNeRF/warped_22/images &    52.8 $\pm$ 0.3 \\
                                              ToRF_Results/VideoNeRF/warped_24/images &    58.9 $\pm$ 0.3 \\
                                              ToRF_Results/VideoNeRF/warped_26/images &    49.3 $\pm$ 0.5 \\

\bottomrule
\end{tabular}

==> figures/raw_brisque_2.tex <==
\begin{tabular}{ll}
\toprule
                                                 filename & BRISQUE_score \\
\midrule

% MP4s for RGB
                                                          filename & BRISQUE_score \\

           ToRF_Results/VideoNeRF_Jul23/quant/dino/video_0_449.mp4 &  10.2$\pm$1.4 \\
    ToRF_Results/VideoNeRF_Jul23/quant/dino_nowrap/video_0_449.mp4 &   7.0$\pm$2.1 \\
      ToRF_Results/VideoNeRF_Jul23/spiral/cupboard/video_0_449.mp4 &  23.2$\pm$3.3 \\
       ToRF_Results/VideoNeRF_Jul23/spiral/deskbox/video_0_449.mp4 &  33.4$\pm$1.9 \\
          ToRF_Results/VideoNeRF_Jul23/spiral/dino/video_0_449.mp4 &  12.0$\pm$2.7 \\
   ToRF_Results/VideoNeRF_Jul23/spiral/dino_nowrap/video_0_449.mp4 &   6.7$\pm$2.6 \\
    ToRF_Results/VideoNeRF_Jul23/spiral/dishwasher/video_0_449.mp4 &  20.1$\pm$2.3 \\
    ToRF_Results/VideoNeRF_Jul23/spiral/phonebooth/video_0_449.mp4 &  31.7$\pm$1.6 \\
   ToRF_Results/VideoNeRF_Jul23/spiral/photocopier/video_0_449.mp4 &  27.1$\pm$1.8 \\
     ToRF_Results/VideoNeRF_Jul23/spiral/studybook/video_0_449.mp4 &  27.2$\pm$1.3 \\

% Time freeze
   ToRF_Results/VideoNeRF_Jul23/spiral_15/cupboard/video_0_449.mp4 &  22.3$\pm$1.7 \\
    ToRF_Results/VideoNeRF_Jul23/spiral_15/deskbox/video_0_449.mp4 &  34.3$\pm$1.4 \\
       ToRF_Results/VideoNeRF_Jul23/spiral_15/dino/video_0_449.mp4 &  13.4$\pm$1.8 \\
ToRF_Results/VideoNeRF_Jul23/spiral_15/dino_nowrap/video_0_449.mp4 &   6.2$\pm$1.1 \\
 ToRF_Results/VideoNeRF_Jul23/spiral_15/dishwasher/video_0_449.mp4 &  19.6$\pm$1.7 \\
 ToRF_Results/VideoNeRF_Jul23/spiral_15/phonebooth/video_0_449.mp4 &  32.1$\pm$1.4 \\
ToRF_Results/VideoNeRF_Jul23/spiral_15/photocopier/video_0_449.mp4 &  27.3$\pm$1.8 \\
  ToRF_Results/VideoNeRF_Jul23/spiral_15/studybook/video_0_449.mp4 &  26.9$\pm$1.1 \\

% Disparity
            ToRF_Results/VideoNeRF_Jul23/quant/dino/disp_0_449.mp4 &  48.3$\pm$2.8 \\
     ToRF_Results/VideoNeRF_Jul23/quant/dino_nowrap/disp_0_449.mp4 &  31.4$\pm$3.5 \\
       ToRF_Results/VideoNeRF_Jul23/spiral/cupboard/disp_0_449.mp4 &  24.5$\pm$2.9 \\
        ToRF_Results/VideoNeRF_Jul23/spiral/deskbox/disp_0_449.mp4 &  48.7$\pm$2.5 \\
           ToRF_Results/VideoNeRF_Jul23/spiral/dino/disp_0_449.mp4 &  46.6$\pm$4.8 \\
    ToRF_Results/VideoNeRF_Jul23/spiral/dino_nowrap/disp_0_449.mp4 &  31.7$\pm$2.4 \\
     ToRF_Results/VideoNeRF_Jul23/spiral/dishwasher/disp_0_449.mp4 &  41.7$\pm$2.0 \\
     ToRF_Results/VideoNeRF_Jul23/spiral/phonebooth/disp_0_449.mp4 &  38.1$\pm$8.2 \\
    ToRF_Results/VideoNeRF_Jul23/spiral/photocopier/disp_0_449.mp4 &  46.5$\pm$7.7 \\
      ToRF_Results/VideoNeRF_Jul23/spiral/studybook/disp_0_449.mp4 &  42.2$\pm$3.3 \\

% Time freeze
    ToRF_Results/VideoNeRF_Jul23/spiral_15/cupboard/disp_0_449.mp4 &  24.2$\pm$2.5 \\
     ToRF_Results/VideoNeRF_Jul23/spiral_15/deskbox/disp_0_449.mp4 &  49.7$\pm$1.5 \\
        ToRF_Results/VideoNeRF_Jul23/spiral_15/dino/disp_0_449.mp4 &  45.5$\pm$3.0 \\
 ToRF_Results/VideoNeRF_Jul23/spiral_15/dino_nowrap/disp_0_449.mp4 &  32.4$\pm$1.3 \\
  ToRF_Results/VideoNeRF_Jul23/spiral_15/dishwasher/disp_0_449.mp4 &  42.8$\pm$2.0 \\
  ToRF_Results/VideoNeRF_Jul23/spiral_15/phonebooth/disp_0_449.mp4 &  35.9$\pm$6.9 \\
 ToRF_Results/VideoNeRF_Jul23/spiral_15/photocopier/disp_0_449.mp4 &  46.8$\pm$5.4 \\
   ToRF_Results/VideoNeRF_Jul23/spiral_15/studybook/disp_0_449.mp4 &  42.6$\pm$2.6 \\


% PNGs RGB
           ToRF_Results/VideoNeRF_Jul23/quant/dino/images &  13.4$\pm$1.6 \\
    ToRF_Results/VideoNeRF_Jul23/quant/dino_nowrap/images &   8.9$\pm$2.2 \\
      ToRF_Results/VideoNeRF_Jul23/spiral/cupboard/images &  27.4$\pm$3.3 \\
       ToRF_Results/VideoNeRF_Jul23/spiral/deskbox/images &  40.3$\pm$1.8 \\
          ToRF_Results/VideoNeRF_Jul23/spiral/dino/images &  15.2$\pm$3.2 \\
   ToRF_Results/VideoNeRF_Jul23/spiral/dino_nowrap/images &   9.2$\pm$2.9 \\
    ToRF_Results/VideoNeRF_Jul23/spiral/dishwasher/images &  24.2$\pm$2.1 \\
    ToRF_Results/VideoNeRF_Jul23/spiral/phonebooth/images &  38.7$\pm$1.3 \\
   ToRF_Results/VideoNeRF_Jul23/spiral/photocopier/images &  34.6$\pm$2.0 \\
     ToRF_Results/VideoNeRF_Jul23/spiral/studybook/images &  34.6$\pm$1.4 \\
   
   ToRF_Results/VideoNeRF_Jul23/spiral_15/cupboard/images &  26.4$\pm$1.7 \\
    ToRF_Results/VideoNeRF_Jul23/spiral_15/deskbox/images &  41.2$\pm$1.1 \\
       ToRF_Results/VideoNeRF_Jul23/spiral_15/dino/images &  16.7$\pm$1.7 \\
ToRF_Results/VideoNeRF_Jul23/spiral_15/dino_nowrap/images &   8.5$\pm$1.3 \\
 ToRF_Results/VideoNeRF_Jul23/spiral_15/dishwasher/images &  23.7$\pm$1.7 \\
 ToRF_Results/VideoNeRF_Jul23/spiral_15/phonebooth/images &  38.7$\pm$1.4 \\
ToRF_Results/VideoNeRF_Jul23/spiral_15/photocopier/images &  35.1$\pm$1.9 \\
  ToRF_Results/VideoNeRF_Jul23/spiral_15/studybook/images &  34.3$\pm$1.2 \\
         
         
% Old numbers at NeurIPS submission time

% MP4s
         ToRF_Results/VideoNeRF_May28/dino_dynamic/video_0_449.mp4 &  48.4$\pm$1.5 \\
           ToRF_Results/VideoNeRF_May28/dishwasher/video_0_449.mp4 &  31.2$\pm$0.8 \\
            ToRF_Results/VideoNeRF_May28/spiral/21/video_0_449.mp4 &  44.9$\pm$1.4 \\
            ToRF_Results/VideoNeRF_May28/spiral/22/video_0_449.mp4 &  41.1$\pm$1.4 \\
            ToRF_Results/VideoNeRF_May28/spiral/25/video_0_449.mp4 &  36.5$\pm$1.6 \\
            ToRF_Results/VideoNeRF_May28/spiral/26/video_0_449.mp4 &  34.2$\pm$1.2 \\
          ToRF_Results/VideoNeRF_May28/spiral/dino/video_0_449.mp4 &  37.7$\pm$1.5 \\
      ToRF_Results/VideoNeRF_May28/spiral/dino-bak/video_0_449.mp4 &  37.7$\pm$1.6 \\
    ToRF_Results/VideoNeRF_May28/spiral/dishwasher/video_0_449.mp4 &  27.6$\pm$1.1 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/21/video_0_449.mp4 &  45.6$\pm$1.1 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/22/video_0_449.mp4 &  41.6$\pm$1.1 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/24/video_0_449.mp4 &  45.9$\pm$0.8 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/25/video_0_449.mp4 &  37.2$\pm$0.8 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/26/video_0_449.mp4 &  34.5$\pm$0.8 \\
       ToRF_Results/VideoNeRF_May28/spiral_15/dino/video_0_449.mp4 &  37.8$\pm$1.7 \\
   ToRF_Results/VideoNeRF_May28/spiral_15/dino-bak/video_0_449.mp4 &  37.8$\pm$1.7 \\
 ToRF_Results/VideoNeRF_May28/spiral_15/dishwasher/video_0_449.mp4 &  28.2$\pm$1.0 \\
            ToRF_Results/VideoNeRF_May28/warped_21/video_0_449.mp4 &  48.7$\pm$0.6 \\
            ToRF_Results/VideoNeRF_May28/warped_22/video_0_449.mp4 &  44.6$\pm$0.5 \\
            ToRF_Results/VideoNeRF_May28/warped_24/video_0_449.mp4 &  49.4$\pm$0.6 \\
            ToRF_Results/VideoNeRF_May28/warped_26/video_0_449.mp4 &  41.6$\pm$0.7 \\

% disparity
          ToRF_Results/VideoNeRF_May28/dino_dynamic/disp_0_449.mp4 &  52.2$\pm$1.4 \\
            ToRF_Results/VideoNeRF_May28/dishwasher/disp_0_449.mp4 &  54.0$\pm$1.0 \\
             ToRF_Results/VideoNeRF_May28/spiral/21/disp_0_449.mp4 &  51.1$\pm$4.6 \\
             ToRF_Results/VideoNeRF_May28/spiral/22/disp_0_449.mp4 &  61.2$\pm$5.4 \\
             ToRF_Results/VideoNeRF_May28/spiral/24/disp_0_449.mp4 &  62.8$\pm$2.1 \\
             ToRF_Results/VideoNeRF_May28/spiral/25/disp_0_449.mp4 &  55.3$\pm$2.0 \\
             ToRF_Results/VideoNeRF_May28/spiral/26/disp_0_449.mp4 &  42.6$\pm$1.9 \\
           ToRF_Results/VideoNeRF_May28/spiral/dino/disp_0_449.mp4 &  54.1$\pm$1.3 \\
       ToRF_Results/VideoNeRF_May28/spiral/dino-bak/disp_0_449.mp4 &  54.1$\pm$1.4 \\
     ToRF_Results/VideoNeRF_May28/spiral/dishwasher/disp_0_449.mp4 &  54.4$\pm$1.4 \\
          ToRF_Results/VideoNeRF_May28/spiral_15/21/disp_0_449.mp4 &  51.5$\pm$6.8 \\
          ToRF_Results/VideoNeRF_May28/spiral_15/22/disp_0_449.mp4 &  60.5$\pm$5.3 \\
          ToRF_Results/VideoNeRF_May28/spiral_15/24/disp_0_449.mp4 &  62.9$\pm$1.2 \\
          ToRF_Results/VideoNeRF_May28/spiral_15/25/disp_0_449.mp4 &  56.6$\pm$2.2 \\
          ToRF_Results/VideoNeRF_May28/spiral_15/26/disp_0_449.mp4 &  42.9$\pm$1.8 \\
        ToRF_Results/VideoNeRF_May28/spiral_15/dino/disp_0_449.mp4 &  54.2$\pm$1.2 \\
    ToRF_Results/VideoNeRF_May28/spiral_15/dino-bak/disp_0_449.mp4 &  54.2$\pm$1.2 \\
  ToRF_Results/VideoNeRF_May28/spiral_15/dishwasher/disp_0_449.mp4 &  55.1$\pm$1.2 \\
             ToRF_Results/VideoNeRF_May28/warped_21/disp_0_449.mp4 &  59.2$\pm$5.8 \\
             ToRF_Results/VideoNeRF_May28/warped_22/disp_0_449.mp4 &  63.8$\pm$1.4 \\
             ToRF_Results/VideoNeRF_May28/warped_24/disp_0_449.mp4 &  64.0$\pm$0.6 \\
             ToRF_Results/VideoNeRF_May28/warped_26/disp_0_449.mp4 &  44.7$\pm$1.7 \\

% PNGs
         ToRF_Results/VideoNeRF_May28/dino_dynamic/images &  58.1$\pm$1.9 \\
           ToRF_Results/VideoNeRF_May28/dishwasher/images &  34.3$\pm$0.6 \\
            ToRF_Results/VideoNeRF_May28/spiral/21/images &  54.0$\pm$1.2 \\
            ToRF_Results/VideoNeRF_May28/spiral/22/images &  50.6$\pm$1.5 \\
            ToRF_Results/VideoNeRF_May28/spiral/24/images &  53.3$\pm$1.6 \\
            ToRF_Results/VideoNeRF_May28/spiral/25/images &  46.2$\pm$1.6 \\
            ToRF_Results/VideoNeRF_May28/spiral/26/images &  40.7$\pm$0.9 \\
          ToRF_Results/VideoNeRF_May28/spiral/dino/images &  45.9$\pm$1.5 \\
      ToRF_Results/VideoNeRF_May28/spiral/dino-bak/images &  45.9$\pm$1.5 \\
    ToRF_Results/VideoNeRF_May28/spiral/dishwasher/images &  30.0$\pm$1.1 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/21/images &  54.3$\pm$0.9 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/22/images &  50.4$\pm$1.0 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/24/images &  55.3$\pm$0.6 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/25/images &  46.4$\pm$0.9 \\
         ToRF_Results/VideoNeRF_May28/spiral_15/26/images &  41.0$\pm$0.6 \\
       ToRF_Results/VideoNeRF_May28/spiral_15/dino/images &  45.9$\pm$1.7 \\
   ToRF_Results/VideoNeRF_May28/spiral_15/dino-bak/images &  45.9$\pm$1.7 \\
 ToRF_Results/VideoNeRF_May28/spiral_15/dishwasher/images &  30.4$\pm$0.7 \\
            ToRF_Results/VideoNeRF_May28/warped_21/images &  56.8$\pm$0.4 \\
            ToRF_Results/VideoNeRF_May28/warped_22/images &  52.8$\pm$0.3 \\
            ToRF_Results/VideoNeRF_May28/warped_24/images &  58.9$\pm$0.3 \\
            ToRF_Results/VideoNeRF_May28/warped_26/images &  49.3$\pm$0.5 \\
\bottomrule
\end{tabular}


==> tables/table02_quant_dynamic.tex <==
% Sequence names
%
% Synthetic
% - MProbe (static)
% - Bathroom (static)
% - Kitchen (static)

% Synthetic
% - MProbe (dynamic)
% - DinoPear (dynamic)

% iPhone 12
% - Dishwasher (dynamic)

% Tof Rig
% - PhoneBooth (dynamic)
% - Cupboard (dynamic)
% - Photocopier (dynamic)
% - StudyBook (dynamic)
% - Desk1 (dynamic)
% - Desk2 (dynamic)


% \begin{table}[t]
% \caption{\label{tab:quantitative-dynamic}%
% 	\emph{Adding ToF data provides higher quality view synthesis}. We compare our method to two neural dynamic reconstruction methods using the BRISQUE no-reference image quality metric \cite{MittaMB2012}. $^\ddagger$\SeqDinoPear~synthetic. $^\ddagger$\SeqDishwasheriPhone~uses processed LIDAR depth from an iPhone 12 Pro as a comparison sequence instead of ToF phasor image supervision. \emph{Note:} As an opinion aware no-reference metric, these numbers are more suggestive than PSNR, and we recommend viewing our supplemental video in addition.\jt{Missing StudyBook}}
% %\resizebox{\linewidth}{!}{%
% % \setlength{\tabcolsep}{3pt}%
% \centering
% \begin{tabular}{l r r r r r r r}
%     \toprule
%     Method / BRISQUE \tridown & \small\SeqPhoneBooth & \small\SeqCupboard & \small\SeqPhotocopier & \small\SeqDeskBox & \small\SeqStudyBook & \small\SeqDinoPear\!$^\dagger$\hspace{-4pt} & \small\SeqDishwasheriPhone\!$^\ddagger$\hspace{-4pt} \\
%     \midrule
%     %
%     %ToF depth splat                 & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x \\
%     %
%     % NeRF~\cite{MildeSTBRN2020}      & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x & xx.x $\pm$ x.x \\
%     % %
%     % VideoNeRF as submitted to NeurIPS (2x input resolution)
%     %VideoNeRF~\cite{XianHKK2021}    & 47.4 $\pm$ 1.1 & 34.2 $\pm$ 1.2 & 41.1 $\pm$ 1.4 & 43.5 $\pm$ 1.8 & 27.6 $\pm$ 1.1 \\
%     % 
%     % VideoNeRF as of July 23rd with correct input size
%     VideoNeRF~\cite{XianHKK2021}    & 38.7 $\pm$ 1.3 & 27.4 $\pm$ 3.3 & 34.6 $\pm$ 2.0 & 40.3 $\pm$ 1.8 & & & 24.2 $\pm$ 2.1 \\
%     % 
%     NSFF~\cite{LiNSW2021}           & 39.9 $\pm$ 1.8 & 35.1 $\pm$ 4.5 & 37.7 $\pm$ 2.6 & 38.5 $\pm$ 3.7 & & & 25.4 $\pm$ 2.8 \\
%     %
%     \midrule
%     \torf (ours)                    & 31.9 $\pm$ 1.3 & 27.2 $\pm$ 3.3 & 30.6 $\pm$ 2.1 & 32.6 $\pm$ 1.9 & & & 25.8 $\pm$ 1.9 \\
%     \bottomrule
% \end{tabular}%
% %}
% \end{table}

% 2021-08-11 - James Tompkin
% Created from MP4 RGB numbers for BRISQUE as this was the only consistent set we had. Not PNGs as some were missing.
% See files raw_brisque.tex and raw_brisque_2.tex for numbers. In figure4_ folder
%
\begin{table}[t]
\caption{
	\emph{Adding ToF data provides higher quality view synthesis}. We compare our method to two neural dynamic reconstruction methods using the BRISQUE no-reference image quality metric~\citep{MittaMB2012}. These are computed over a spiral of novel views at the \nth{15} frame per sequence. $^\ddagger$\SeqDinoPear~is synthetic. $^\ddagger$\SeqDishwasheriPhone~uses processed LIDAR depth from an iPhone 12 Pro as a comparison sequence instead of ToF phasor image supervision. \emph{Note:} As an opinion-aware no-reference metric, these numbers are more suggestive than PSNR; please view our supplemental videos. \TODO{recompute}
	}
\label{tab:quantitative-dynamic}
%\resizebox{\linewidth}{!}{%
% \setlength{\tabcolsep}{3pt}%
\centering
\begin{tabular}{l r r r}
    \toprule
    Seq.~/ BRISQUE \tridown & VideoNeRF~\cite{XianHKK2021} & NSFF~\cite{LiNSW2021} & \torf (ours) \\
    \midrule
    
    \SeqPhoneBooth  & 37.7$\pm$1.6    & 40.6$\pm$2.5    & 33.8$\pm$2.1 \\
    \SeqCupboard    & 25.2$\pm$3.5    & 30.1$\pm$3.9    & 30.4$\pm$2.6 \\
    \SeqPhotocopier & 34.7$\pm$2.5    & 40.6$\pm$4.7    & 36.5$\pm$1.8 \\
    \SeqDeskBox     & 38.7$\pm$1.4    & 37.3$\pm$2.3    & 38.0$\pm$2.9 \\
    \SeqStudyBook   & 34.6$\pm$1.7    & 34.5$\pm$1.8    & 34.9$\pm$1.8 \\
    \midrule
    %\SeqDinoPear\!$^\dagger$\hspace{-4pt}           & 13.4 $\pm$ 1.8    & 21.9 $\pm$ 3.3    & 18.8 $\pm$ 1.7 \\ 
    \SeqDishwasheriPhone\!$^\ddagger$\hspace{-4pt}  & 28.9$\pm$1.5    & 19.7$\pm$2.5    & 26.6$\pm$1.1 \\
    \midrule
    Mean avg.~      & 31.6 $\pm$ 2.0    & 33.8 $\pm$ 2.9    & 33.4 $\pm$ 2.0 \\
    \bottomrule
\end{tabular}%
%}
\end{table}
